Radio SLAM for 6G Systems at THz Frequencies: Design and Experimental Validation

Next-generation wireless networks will see the convergence of communication and sensing, also exploiting the availability of large bandwidths in the Terahertz (THz) spectrum and electrically large antenna arrays on handheld devices. In particular, it is envisaged that user devices will be able to automatically scan their surroundings by steering a very narrow antenna beam and collecting echoes reflected by objects and walls to derive a map of indoors and infer users' trajectories using simultaneous localization and mapping (SLAM) techniques. In this paper, we address this scenario by proposing original radioSLAM (R-SLAM) algorithms, derived from image processing techniques, to map the environment and pinpoint the device position in the map starting from measurements sensed by a mobile THz radar. Initially, to fully understand the THz backscattering phenomenon, we provide an experimental characterization of the THz backscattering channel in indoor environments. Then, the performance of the proposed algorithms is assessed using real-world THz radar measurements and is compared with state-of-the-art SLAM techniques, demonstrating the superiority of the proposed approaches.

==> Radio SLAM_submitted/Figures/FourierMellin.tex <==


\tikzset{every picture/.style={line width=0.75pt,font=\small}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.6pt,y=0.6pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,323); %set diagram left start at 0, and has height of 323

%Shape: Rectangle [id:dp10677334533740424] 
\draw  [fill={rgb, 255:red, 247; green, 235; blue, 255 }  ,fill opacity=1 ] (135.5,59.75) -- (269.5,59.75) -- (269.5,94.75) -- (135.5,94.75) -- cycle ;

%Shape: Rectangle [id:dp6359939704896505] 
\draw  [fill={rgb, 255:red, 247; green, 235; blue, 255 }  ,fill opacity=1 ] (295.5,59.75) -- (395.5,59.75) -- (395.5,94.75) -- (295.5,94.75) -- cycle ;

%Shape: Rectangle [id:dp8670183385211978] 
\draw  [fill={rgb, 255:red, 247; green, 235; blue, 255 }  ,fill opacity=1 ] (421.5,59.75) -- (521.5,59.75) -- (521.5,94.75) -- (421.5,94.75) -- cycle ;

%Shape: Rectangle [id:dp40872659892674545] 
\draw  [fill={rgb, 255:red, 247; green, 235; blue, 255 }  ,fill opacity=1 ] (547.5,59.75) -- (681.5,59.75) -- (681.5,94.75) -- (547.5,94.75) -- cycle ;

%Straight Lines [id:da2472011626412518] 
\draw    (274,77.38) -- (289,77.15) ;
\draw [shift={(291,77.13)}, rotate = 179.16] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da27927527169106336] 
\draw    (400,77.38) -- (415,77.15) ;
\draw [shift={(417,77.13)}, rotate = 179.16] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da1365268653122944] 
\draw    (526,77.38) -- (541,77.15) ;
\draw [shift={(543,77.13)}, rotate = 179.16] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Rectangle [id:dp18905477156185801] 
\draw  [fill={rgb, 255:red, 247; green, 235; blue, 255 }  ,fill opacity=1 ] (135.5,121.75) -- (269.5,121.75) -- (269.5,156.75) -- (135.5,156.75) -- cycle ;

%Shape: Rectangle [id:dp7493271736252769] 
\draw  [fill={rgb, 255:red, 247; green, 235; blue, 255 }  ,fill opacity=1 ] (295.5,121.75) -- (395.5,121.75) -- (395.5,156.75) -- (295.5,156.75) -- cycle ;

%Shape: Rectangle [id:dp7010940599585422] 
\draw  [fill={rgb, 255:red, 247; green, 235; blue, 255 }  ,fill opacity=1 ] (421.5,121.75) -- (521.5,121.75) -- (521.5,156.75) -- (421.5,156.75) -- cycle ;

%Shape: Rectangle [id:dp056754669145771874] 
\draw  [fill={rgb, 255:red, 247; green, 235; blue, 255 }  ,fill opacity=1 ] (547.5,121.75) -- (681.5,121.75) -- (681.5,156.75) -- (547.5,156.75) -- cycle ;

%Straight Lines [id:da9179324564136195] 
\draw    (274,139.38) -- (289,139.15) ;
\draw [shift={(291,139.13)}, rotate = 179.16] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da666519541402383] 
\draw    (400,139.38) -- (415,139.15) ;
\draw [shift={(417,139.13)}, rotate = 179.16] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da5982289134867569] 
\draw    (526,139.38) -- (541,139.15) ;
\draw [shift={(543,139.13)}, rotate = 179.16] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Shape: Rectangle [id:dp6493555873953609] 
\draw  [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,draw opacity=1 ][dash pattern={on 4.5pt off 4.5pt}] (710.5,60) -- (799.5,60) -- (799.5,156.75) -- (710.5,156.75) -- cycle ;

%Shape: Rectangle [id:dp02690770280662802] 
\draw  [fill={rgb, 255:red, 0; green, 255; blue, 0 }  ,fill opacity=0.2 ] (211,187.5) -- (379,187.5) -- (379,222.5) -- (211,222.5) -- cycle ;

%Shape: Rectangle [id:dp6425816540596738] 
\draw  [fill={rgb, 255:red, 0; green, 255; blue, 0 }  ,fill opacity=0.2 ] (497,235.5) -- (660,235.5) -- (660,293) -- (497,293) -- cycle ;
%Straight Lines [id:da78120706358774] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 255 }  ,draw opacity=1 ]   (233,253.5) -- (300,253.5) ;
\draw [shift={(302,253.5)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 255 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Rectangle [id:dp867858569358271] 
\draw  [fill={rgb, 255:red, 247; green, 235; blue, 255 }  ,fill opacity=1 ] (308,245.5) -- (442,245.5) -- (442,280.5) -- (308,280.5) -- cycle ;

%Straight Lines [id:da21600648402401434] 
\draw    (667,261.5) -- (689,261.96) ;
\draw [shift={(691,262)}, rotate = 181.19] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da3551238949176303] 
\draw    (99.5,274) -- (300.5,274) ;
\draw [shift={(302.5,274)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da8996582682982741] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 255 }  ,draw opacity=1 ]   (90.5,191) -- (202.5,191) ;
\draw [shift={(204.5,191)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 255 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da9711597201841378] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 255 }  ,draw opacity=1 ]   (814.5,193) -- (384,193) ;
\draw [shift={(382,193)}, rotate = 360] [color={rgb, 255:red, 0; green, 0; blue, 255 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da07065715411446116] 
\draw    (448,273) -- (490,273) ;
\draw [shift={(492,273)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da4141983392253823] 
\draw [color={rgb, 255:red, 0; green, 22; blue, 255 }  ,draw opacity=1 ]   (233,228.5) -- (233,253.5) ;
%Straight Lines [id:da5575693802139814] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 255 }  ,draw opacity=1 ]   (448,253) -- (490,253) ;
\draw [shift={(492,253)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 255 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da060849464608569326] 
\draw    (808,99.5) -- (830,99.96) ;
\draw [shift={(832,100)}, rotate = 181.19] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da8133765397443635] 
\draw    (91,77.13) -- (127,77.13) ;
\draw [shift={(129,77.13)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da3718153490478837] 
\draw    (83,140) -- (119,140) ;
\draw [shift={(121,140)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da08897125933103323] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 255 }  ,draw opacity=1 ]   (90.5,139.5) -- (90.5,191) ;
%Straight Lines [id:da40805831879717247] 
\draw    (101.5,77.5) -- (99.5,274) ;
%Straight Lines [id:da40630061808367657] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 255 }  ,draw opacity=1 ]   (814.5,99.5) -- (814.5,193) ;
%Straight Lines [id:da4249920097278328] 
\draw    (686.5,76.38) -- (701.5,76.15) ;
\draw [shift={(703.5,76.13)}, rotate = 179.16] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da8727419100886242] 
\draw    (686.5,140.38) -- (701.5,140.15) ;
\draw [shift={(703.5,140.13)}, rotate = 179.16] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

% Text Node
\draw (157,68.75) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\left(\rho, \theta \right) \rightarrow (x,y)$};
% Text Node
\draw (454,68.75) node [anchor=north west][inner sep=0.75pt]   [align=left] {Magn.};
% Text Node
\draw (318.5,67.25) node [anchor=north west][inner sep=0.75pt]   [align=left] {2D-FFT};
% Text Node
\draw (570,68.75) node [anchor=north west][inner sep=0.75pt]   [align=left] {$(x,y) \rightarrow \left(\rho, \theta \right)$};
% Text Node
\draw (570,130.75) node [anchor=north west][inner sep=0.75pt]   [align=left] {$(x,y) \rightarrow \left(\rho, \theta \right)$};
% Text Node
\draw (454,130.75) node [anchor=north west][inner sep=0.75pt]   [align=left] {Magn.};
% Text Node
\draw (318.5,129.25) node [anchor=north west][inner sep=0.75pt]   [align=left] {2D-FFT};
% Text Node
\draw (157,130.75) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\left(\rho, \theta \right) \rightarrow (x,y)$};
% Text Node
\draw (755.18,108.38) node  [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,opacity=1 ] [align=left] {Rotation \\Angle\\Estimator};
% Text Node
\draw (697,252.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\tilde{dx}$, $\tilde{dy}$};
% Text Node
\draw (513,245.25) node [anchor=north west][inner sep=0.75pt]   [align=center] {\begin{minipage}[lt]{90.6pt}\setlength\topsep{0pt}
\begin{center}
\!\!\!\!\!\!\!\!\!\!\!\! Translational Offset\\
\!\!\!\!\!\!\!\!Estimator
\end{center}

\end{minipage}};
% Text Node
\draw (837,91.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\tilde{d\theta}$};
% Text Node
\draw (58,66) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\mathbf{F}_k$};
% Text Node
\draw (40,131) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\mathbf{F}_{k-1}$};
% Text Node
\draw (180,32.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {\textit{Step 1}};
% Text Node
\draw (323,32.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {\textit{Step 2}};
% Text Node
\draw (449,32.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {\textit{Step 3}};
% Text Node
\draw (592,32.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {\textit{Step 4}};
% Text Node
\draw (722,32.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {\textit{Steps 5-8}};
% Text Node
\draw (272.5,165) node [anchor=north west][inner sep=0.75pt]   [align=left] {\textit{Step 9}};
% Text Node
\draw (348,287) node [anchor=north west][inner sep=0.75pt]   [align=left] {\textit{Step 10}};
% Text Node
\draw (552,299) node [anchor=north west][inner sep=0.75pt]   [align=left] {\textit{Step 11}};
% Text Node
\draw (320,254.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\left(\rho, \theta \right) \rightarrow (x,y)$};
% Text Node
\draw (215.5,196.5) node [anchor=north west][inner sep=0.75pt]   [align=center] {\,\,\,Rotation Compensation};


\end{tikzpicture}

==> Radio SLAM_submitted/Figures/ProcessingChain_2.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\tikzset{
  font={\fontsize{7pt}{12}\selectfont}}
  
\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-0.6,xscale=0.6]
%uncomment if require: \path (0,230); %set diagram left start at 0, and has height of 230

%Shape: Rectangle [id:dp7305623848140894] 
\draw  [fill={rgb, 255:red, 0; green, 255; blue, 0 }  ,fill opacity=0.2 ] (106,97.5) -- (167,97.5) -- (167,132.5) -- (106,132.5) -- cycle ;

%Shape: Rectangle [id:dp17953923979748732] 
\draw  [fill={rgb, 255:red, 10; green, 100; blue, 255 }  ,fill opacity=0.2] (203,85.5) -- (293,85.5) -- (293,144) -- (203,144) -- cycle ;
%Shape: Rectangle [id:dp464327684389654] 
\draw  [fill={rgb, 255:red, 10; green, 100; blue, 255 }  ,fill opacity=0.2] (330,85.5) -- (420,85.5) -- (420,144) -- (330,144) -- cycle ;
%Shape: Rectangle [id:dp211782835478326] 
\draw  [fill={rgb, 255:red, 10; green, 100; blue, 255 }  ,fill opacity=0.2 ] (458,96.75) -- (569,96.75) -- (569,132.75) -- (458,132.75) -- cycle ;
%Shape: Rectangle [id:1 frame delay] 
\draw  [fill={rgb, 255:red, 248; green, 221; blue, 251 }  ,fill opacity=1 ] (662,21) -- (774,21) -- (774,58) -- (662,58) -- cycle ;
%Shape: Rectangle [id:Pose Estimation] 
\draw  [fill={rgb, 255:red, 248; green, 221; blue, 251 }  ,fill opacity=1 ] (662,85.5) -- (752,85.5) -- (752,144) -- (662,144) -- cycle ;
%Shape: Rectangle [id:Kalman Filter] 
\draw  [fill={rgb, 255:red, 248; green, 221; blue, 251 }  ,fill opacity=1 ] (859,32.31) -- (949,32.31) -- (949,90.81) -- (859,90.81) -- cycle ;
%Shape: Rectangle [id:Mapping] 
\draw  [fill={rgb, 255:red, 248; green, 221; blue, 251 }  ,fill opacity=1 ] (860,143) -- (950,143) -- (950,179) -- (860,179) -- cycle ;


%Shape: Boxed Polygon [id:dp6838979827260208] 
\draw  [color={rgb, 255:red, 126; green, 211; blue, 33 }  ,draw opacity=1 ][line width=0.75]  (84.75,111.1) -- (101.5,111.1) -- (101.5,113.87) -- (84.31,113.87) -- (75.5,120.64) -- (75.5,104.64) -- cycle ;
%Shape: Boxed Polygon [id:dp4720442985185693] 
\draw  [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][dash pattern={on 1.5pt off 1.5pt on 1.5pt off 1.5pt}][line width=0.75]  (85.73,95.32) -- (100.96,102.29) -- (99.81,104.81) -- (84.18,97.65) -- (73.35,100.14) -- (80.01,85.59) -- cycle ;
%Shape: Boxed Polygon [id:dp0029086877964439317] 
\draw  [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][dash pattern={on 1.5pt off 1.5pt on 1.5pt off 1.5pt}][line width=0.75]  (85.73,129.96) -- (100.96,122.99) -- (99.81,120.47) -- (84.18,127.62) -- (73.35,125.14) -- (80.01,139.69) -- cycle ;

%Straight Lines [id:da4640710012586746] 
\draw [color={rgb, 255:red, 126; green, 211; blue, 33 }  ,draw opacity=1 ]   (71,113.5) -- (35,113.5) ;
\draw [shift={(33,113.5)}, rotate = 360] [color={rgb, 255:red, 126; green, 211; blue, 33 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da455638582362736] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ] [dash pattern={on 4.5pt off 4.5pt}]  (72.73,90.32) -- (43.66,70.62) ;
\draw [shift={(42,69.5)}, rotate = 34.11] [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da8899315454681116] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ] [dash pattern={on 4.5pt off 4.5pt}]  (72.73,135.32) -- (40.58,148.56) ;
\draw [shift={(38.73,149.32)}, rotate = 337.62] [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;


%Straight Lines [id:da7919015457015264] 
\draw    (172,116.38) -- (195,116.03) ;
\draw [shift={(197,116)}, rotate = 179.14] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da19011467541463256] 
\draw    (298,114.94) -- (321,114.59) ;
\draw [shift={(323,114.56)}, rotate = 179.14] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da35223384127908974] 
\draw    (426,114.94) -- (449,114.59) ;
\draw [shift={(451,114.56)}, rotate = 179.14] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da7833156998196] 
\draw    (573,114.75) -- (646,114.75) ;
\draw [shift={(648,114.75)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da34027701015716594] 
%\draw    (762,114.75) -- (852,114.75) ;
%\draw [shift={(854,114.75)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da15588280655290854] 
%\draw    (964,110.38) -- (987,110.03) ;
%\draw [shift={(989,110)}, rotate = 179.14] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da10482767150232108] 
%\draw    (964,184.38) -- (987,184.03) ;
%\draw [shift={(989,184)}, rotate = 179.14] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da7803181825334069] 
\draw    (706,61) -- (706,77.5) ;
\draw [shift={(706,79.5)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Rectangle [id:dp6372042761950347] 
\draw  [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][dash pattern={on 4.5pt off 4.5pt}] (198,-70) -- (623,-70) -- (623,187.5) -- (198,187.5) -- cycle ;

%Shape: Rectangle [id:dp05145868463146819] 
\draw  [color={rgb, 255:red, 189; green, 16; blue, 224 }  ,draw opacity=1 ][dash pattern={on 4.5pt off 4.5pt}] (650,15.06) -- (966,15.06) -- (966,214.06) -- (650,214.06) -- cycle ;

%Shape: Rectangle [id:dp4057028950747741] 
\draw  [fill={rgb, 255:red, 248; green, 221; blue, 251 }  ,fill opacity=1 ] (777,100.31) -- (832,100.31) -- (832,127.81) -- (777,127.81) -- cycle ;


%Straight Lines [id:da3514179341560604] 
\draw    (755,114.56) -- (770,114.56) ;
\draw [shift={(772,114.56)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da7683418163963038] 
%\draw    (835,114.56) -- (856,114.56) ;
%\draw [shift={(858,114.56)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da7387402711005613] 
%\draw    (906,144) -- (906,160.5) ;
%\draw [shift={(906,162.5)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:input mapping] 
\draw    (631,114.5) -- (631,160.5) ;
%Straight Lines [id:da9349204571514125] 
%\draw    (631,160.5) -- (837,160.5) ;
\draw    (631,160.5) -- (850,160.5) ;
\draw [shift={(852,160.5)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da09075929940455629] 
%\draw    (837,160.5) -- (837,185.5) ;
%Straight Lines [id:da8485100182765464] 
%\draw    (837,185.5) -- (851,185.5) ;
%\draw [shift={(853,185.5)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da5684796655652049] 
\draw    (631,40) -- (631,114.5) ;
%Straight Lines [id:input di 1 frame delay] 
\draw    (631,40) -- (645,40) ;
\draw [shift={(647,40)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Image [id:dp5304610400367669] 
\draw (1042,110) node  {\includegraphics[width=43pt,height=43pt]{Figures/maptraj.png}};
%Image [id:dp9421609577647383] 
\draw (310.5,0) node  {\includegraphics[width=30pt,height=54pt]{Figures/Fnoclean.png}};
%Image [id:dp8630539854448116] 
\draw (560.5,0) node  {\includegraphics[width=30pt,height=54pt]{Figures/Fclean.png}};

% Text Node
\draw (115,106.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {Radar};
% Text Node
\draw (1030,43) node   [align=left] {\begin{minipage}[lt]{105pt}\setlength\topsep{0pt}
\begin{center}
Trajectory Estimate
\end{center}

\end{minipage}};
% Text Node 
\draw (1015,181) node   [align=left] {\begin{minipage}[lt]{45pt}\setlength\topsep{0pt}
\begin{center}
Map Estimate
\end{center}

\end{minipage}};
% Text Node
\draw (722,190) node   [align=left] {\begin{minipage}[lt]{90.22pt}\setlength\topsep{0pt}
\begin{center}
\textcolor[rgb]{0.74,0.06,0.88}{Trajectory and Map}
\end{center}
\end{minipage}};
\draw (722,202) node   [align=left] {\begin{minipage}[lt]{90.22pt}\setlength\topsep{0pt}
\begin{center}
\textcolor[rgb]{0.74,0.06,0.88}{Estimation}
\end{center}
\end{minipage}};

% Text Node
%\draw (806,98) node   [align=left] {\begin{minipage}[lt]{65.66pt}\setlength\topsep{0pt}
%\begin{center}
% $z_k \rightarrow \mathbf{p}_k$
%\end{center}

%\end{minipage}};
% Text Node
\draw (309,132) node   [align=left] {\begin{minipage}[lt]{10.09pt}\setlength\topsep{0pt}
\begin{center}
$\mathbf{H}$
\end{center}

\end{minipage}};
% Text Node
\draw (598,132) node   [align=left] {\begin{minipage}[lt]{14.63pt}\setlength\topsep{0pt}
\begin{center}
$\mathbf{F}_k$
\end{center}

\end{minipage}};
% Text Node
\draw (23.5,65) node   [align=left] {\begin{minipage}[lt]{14.07pt}\setlength\topsep{0pt}
\begin{center}
$\phi_1$
\end{center}

\end{minipage}};
% Text Node
\draw (23.5,152) node   [align=left] {\begin{minipage}[lt]{14.07pt}\setlength\topsep{0pt}
\begin{center}
$\phi_N$
\end{center}

\end{minipage}};
% Text Node
\draw (263,171) node   [align=left] {\begin{minipage}[lt]{72.45pt}\setlength\topsep{0pt}
\begin{center}
\textcolor[rgb]{0.29,0.56,0.89}{Pre-Processing}
\end{center}

\end{minipage}};
% Text Node
\draw (736,64) node   [align=left] {\begin{minipage}[lt]{14.63pt}\setlength\topsep{0pt}
\begin{center}
$\mathbf{F}_{k-1}$
\end{center}

\end{minipage}};
% Text Node
\draw (260,5) node   [align=left,rotate=90] {\begin{minipage}[lt]{100pt}\setlength\topsep{0pt}
\begin{center}
Angle [$^\circ$]
\end{center}

\end{minipage}};
% Text Node
\draw (510,5) node   [align=left,rotate=90] {\begin{minipage}[lt]{100pt}\setlength\topsep{0pt}
\begin{center}
Angle [$^\circ$]
\end{center}

\end{minipage}};
% Text Node
\draw (310.5,72) node   [align=left] {\begin{minipage}[lt]{100pt}\setlength\topsep{0pt}
\begin{center}
Delay [s]
\end{center}

\end{minipage}};
% Text Node
\draw (557.5,72) node   [align=left] {\begin{minipage}[lt]{100pt}\setlength\topsep{0pt}
\begin{center}
Delay [s]
\end{center}

\end{minipage}};
% Text Node
\draw (248,114.75) node   [align=left] {\begin{minipage}[lt]{58.28pt}\setlength\topsep{0pt}
\begin{center}
Angle-Delay\\Matrix
\end{center}

\end{minipage}};
% Text Node
\draw (375,114.75) node   [align=left] {\begin{minipage}[lt]{58.66pt}\setlength\topsep{0pt}
\begin{center}
Ghost Effect\\Mitigation
\end{center}

\end{minipage}};
% Text Node
\draw (513.5,114.75) node   [align=left] {\begin{minipage}[lt]{69.62pt}\setlength\topsep{0pt}
\begin{center}
Noise Masking
\end{center}

\end{minipage}};
% Text Node
\draw (707,114.75) node   [align=left] {\begin{minipage}[lt]{50.34pt}\setlength\topsep{0pt}
\begin{center}
Relative Pose\\Estimation
\end{center}

\end{minipage}};
% Text Node
\draw (717,39.75) node   [align=left] {\begin{minipage}[lt]{65.08pt}\setlength\topsep{0pt}
\begin{center}
1-frame delay
\end{center}

\end{minipage}};
% Text Node
\draw (904,61.56) node   [align=left] {\begin{minipage}[lt]{37.3pt}\setlength\topsep{0pt}
\begin{center}
Kalman\\Filter
\end{center}

\end{minipage}};
% Text Node
\draw (905,161) node   [align=left] {\begin{minipage}[lt]{41.85pt}\setlength\topsep{0pt}
\begin{center}
Mapping
\end{center}

\end{minipage}};

% Text Node
\draw (804.5,114.56) node   [align=left] {\begin{minipage}[lt]{10.09pt}\setlength\topsep{0pt}
\begin{center}
$\Psi$
\end{center}
\end{minipage}};

% Text Node
\draw (765,100) node   [align=left] {\begin{minipage}[lt]{8.67pt}\setlength\topsep{0pt}
\begin{center}
$\tilde{{\mathbf{z}}}_k$
\end{center}
\end{minipage}};

% Text Node
\draw (823,30) node   [align=left] {\begin{minipage}[lt]{8.67pt}\setlength\topsep{0pt}
\begin{center}
$\hat{\mathbf{p}}_k$
\end{center}

\end{minipage}};

%Straight Lines [id:da4005010179288657] 
\draw    (953,63) -- (982,63) ;
\draw [shift={(984,63)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da45187419961434716] 
\draw    (960.5,63) -- (960.5,110) ;
%Straight Lines [id:da6508049098301798] 
\draw    (910,110) -- (960.5,110) ;
%Straight Lines [id:da7387402711005613] 
\draw    (910,110) -- (910,135) ;
\draw [shift={(910,137)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da3582839386302836] 
\draw    (804,50) -- (804,95) ;
%Straight Lines [id:da7683418163963038] 
\draw    (804,50) -- (851,50.54) ;
\draw [shift={(853,50.56)}, rotate = 180.66] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da6826602173371152] 
\draw    (955,160) -- (984,160) ;
\draw [shift={(986,160)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;


\end{tikzpicture}

==> Radio SLAM_submitted/Figures/SimplifiedFourierMellin.tex <==


\tikzset{every picture/.style={line width=0.75pt,font=\small}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.6pt,y=0.6pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,310); %set diagram left start at 0, and has height of 310

%Shape: Rectangle [id:dp38331830319223825] 
\draw  [fill={rgb, 255:red, 247; green, 235; blue, 255 }  ,fill opacity=1 ] (93,55.5) -- (193,55.5) -- (193,90.5) -- (93,90.5) -- cycle ;
%Shape: Rectangle [id:dp23167463729885696] 
\draw  [fill={rgb, 255:red, 247; green, 235; blue, 255 }  ,fill opacity=1 ] (93,100.5) -- (193,100.5) -- (193,135.5) -- (93,135.5) -- cycle ;
%Shape: Rectangle [id:dp3389305696846927] 
\draw  [fill={rgb, 255:red, 0; green, 255; blue, 0 }  ,fill opacity=0.2 ] (223,51) -- (330,51) -- (330,140) -- (223,140) -- cycle ;
%Shape: Rectangle [id:dp9385230426990023] 
\draw  [fill={rgb, 255:red, 247; green, 235; blue, 255 }  ,fill opacity=1 ] (365,78) -- (465,78) -- (465,113) -- (365,113) -- cycle ;
%Shape: Rectangle [id:dp7664959845090602] 
\draw  [fill={rgb, 255:red, 0; green, 255; blue, 0 }  ,fill opacity=0.2 ] (501,78) -- (601,78) -- (601,113) -- (501,113) -- cycle ;
%Straight Lines [id:da39207377795337894] 
\draw    (470,95.25) -- (492,95.71) ;
\draw [shift={(494,95.75)}, rotate = 181.19] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da40201902037532] 
\draw    (338,95.25) -- (360,95.71) ;
\draw [shift={(362,95.75)}, rotate = 181.19] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da018059119749245456] 
\draw    (194.5,70.75) -- (216.5,71.21) ;
\draw [shift={(218.5,71.25)}, rotate = 181.19] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da8844665988921527] 
\draw    (194.5,119.75) -- (216.5,120.21) ;
\draw [shift={(218.5,120.25)}, rotate = 181.19] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da21220349528678817] 
\draw    (611,95.25) -- (655,95.49) ;
\draw [shift={(657,95.5)}, rotate = 180.31] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da47178380841557255] 
\draw    (30,71) -- (66,71) ;
\draw [shift={(68,71)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da7387409769267257] 
\draw    (31,114) -- (67,114) ;
\draw [shift={(69,114)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Rectangle [id:dp032270465757163525] 
\draw  [fill={rgb, 255:red, 0; green, 255; blue, 0 }  ,fill opacity=0.2] (118,183) -- (286,183) -- (286,218) -- (118,218) -- cycle ;
%Shape: Rectangle [id:dp4434141229775037] 
\draw  [fill={rgb, 255:red, 0; green, 255; blue, 0 }  ,fill opacity=0.2 ] (404,243) -- (567,243) -- (567,300.5) -- (404,300.5) -- cycle ;
%Straight Lines [id:da41745561250830376] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 255 }  ,draw opacity=1 ]   (140,261) -- (207,261) ;
\draw [shift={(209,261)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 255 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Rectangle [id:dp1866822481651227] 
\draw  [fill={rgb, 255:red, 247; green, 235; blue, 255 }  ,fill opacity=1 ] (215,253) -- (349,253) -- (349,288) -- (215,288) -- cycle ;
%Straight Lines [id:da42077441741321686] 
\draw    (574,269) -- (596,269.46) ;
\draw [shift={(598,269.5)}, rotate = 181.19] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Rectangle [id:dp46594242167707467] 
\draw  [color={rgb, 255:red, 245; green, 35; blue, 35 }  ,draw opacity=1 ][dash pattern={on 4.5pt off 4.5pt}][line width=0.75]  (82.5,7) -- (617.5,7) -- (617.5,155.88) -- (82.5,155.88) -- cycle ;
%Straight Lines [id:da15296775759988335] 
\draw    (40,70.5) -- (41,280) ;
%Straight Lines [id:da9861843134358594] 
\draw    (41,280) -- (207,280.49) ;
\draw [shift={(209,280.5)}, rotate = 180.17] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da4218315074720702] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 255 }  ,draw opacity=1 ]   (50,114) -- (51,200.5) ;
%Straight Lines [id:da8916678756777106] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 255 }  ,draw opacity=1 ]   (51,200.5) -- (111,200.5) ;
\draw [shift={(113,200.5)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 255 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da26006080999948544] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 255 }  ,draw opacity=1 ]   (630,99.5) -- (631,199.5) ;
%Straight Lines [id:da8799719257726111] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 255 }  ,draw opacity=1 ]   (631,199.5) -- (291,200.49) ;
\draw [shift={(289,200.5)}, rotate = 359.83] [color={rgb, 255:red, 0; green, 0; blue, 255 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da4584351081078857] 
\draw    (355,280.5) -- (397,280.5) ;
\draw [shift={(399,280.5)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da4440626596802242] 
\draw [color={rgb, 255:red, 0; green, 22; blue, 255 }  ,draw opacity=1 ]   (140,222) -- (140,261) ;
%Straight Lines [id:da14257357296453255] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 255 }  ,draw opacity=1 ]   (355,260.5) -- (397,260.5) ;
\draw [shift={(399,260.5)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 255 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

% Text Node
\draw (116,63) node [anchor=north west][inner sep=0.75pt]   [align=left] {2D-FFT};
% Text Node
\draw (432,13) node [anchor=north west][inner sep=0.75pt]  [color={rgb, 255:red, 255; green, 0; blue, 0 }  ,opacity=1 ] [align=left] {Rotation Angle Estimator};
% Text Node
\draw (636,69) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\tilde{d\theta}$};
% Text Node
\draw (604,260) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\tilde{dx}$,$\tilde{dy}$};
% Text Node
\draw (6,64) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\mathbf{F}_{k}$};
% Text Node
\draw (3,107) node [anchor=north west][inner sep=0.75pt]   [align=left] {\!\!\!\!\! \!\!\!\!\! $\mathbf{F}_{k-1}$};
% Text Node
\draw (322.85,95.5) node [anchor=east] [inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{64.5pt}\setlength\topsep{0pt}
\begin{center}
\quad \, Cross-Power \\\quad \, Spectrum
\end{center}

\end{minipage}};
% Text Node
\draw (415,252.75) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{90.6pt}\setlength\topsep{0pt}
\begin{center}
\!\!\!\!\!\!\!\! Translational Offset\\
\!\!\!\!\!\!\!\!Estimator
\end{center}


\end{minipage}};
% Text Node
\draw (511,87) node [anchor=north west][inner sep=0.75pt]   [align=left] {Max-search};
% Text Node
\draw (122.5,192) node [anchor=north west][inner sep=0.75pt]   [align=left] {\,\,\,Rotation Compensation};
% Text Node
\draw (116,109.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {2D-FFT};
% Text Node
\draw (386,87) node [anchor=north west][inner sep=0.75pt]   [align=left] {2D-IFFT};
% Text Node
\draw (235,262) node [anchor=north west][inner sep=0.75pt]   [align=left] {$(\rho, \theta) \rightarrow (x,y)$};
% Text Node
\draw (120,25) node [anchor=north west][inner sep=0.75pt]   [align=left] {\textit{Step 5}};
% Text Node
\draw (252,25) node [anchor=north west][inner sep=0.75pt]   [align=left] {\textit{Step 6}};
% Text Node
\draw (388,54.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {\textit{Step 7}};
% Text Node
\draw (526,54.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {\textit{Step 8}};


\end{tikzpicture}

==> Radio SLAM_submitted/acronyms.tex <==

%C
\acrodef{CLEAN}{CLEAN}
\acrodef{CFAR}{constant false alarm rate}
\acrodef{CFR}{channel frequency response}
\acrodef{CIR}{channel impulse response}
%G
\acrodef{GEM}{ghost-effect mitigation}
%H
\acrodef{HPBW}{Half Power Beam Width}
%I
\acrodef{IDFT}{inverse discrete Fourier transform}
\acrodef{IFBW}{Intermediate Frequency Band Width}
%L
\acrodef{Lidar}{laser-based radar}
%M
\acrodef{MAP}{maximum a posteriori}
\acrodef{MIMO}{multiple-input multiple-output}
%N
\acrodef{NM}{noise-masking}
%P
\acrodef{pdf}{probability density function}
\acrodef{pmf}{probability mass function}
%R
\acrodef{RIS}{reconfigurable intelligent surface}
\acrodef{RMSE}{root-mean-square error}
\acrodef{R-SLAM}{radio-SLAM}
%S
\acrodef{SLAM}{simultaneous localization and mapping}
%T
\acrodef{THz}{Terahertz}
%U
\acrodef{UAV}{unmanned aerial vehicle}
%V
\acrodef{VNA}{Vector Network Analyzer}
\acrodef{V-SLAM}{Visual-SLAM}
% numbers
\acrodef{5G}{fifth generation}
\acrodef{6G}{sixth generation}
\acrodef{RF}{radio frequency}
\acrodef{psd}{power spectral density}
\acrodef{SFCW}{Stepped-Frequency Continuous-Wave}






==> Radio SLAM_submitted/definitions.tex <==

% Math definition
\newcommand{\tra}{\mathsf{T}}
% Mapping definition
\newcommand{\Ncell}{N_{\mathsf{cell}}}
\newcommand{\map}{\mathbf{m}}
\newcommand{\hmapk}{\hat{\mathbf{m}}_k}
\newcommand{\hmapik}{\hat{m}_{i,k}}
\newcommand{\hmapsk}{\hat{m}_{1,k}}
\newcommand{\hmapek}{\hat{m}_{\Ncell,k}}
\newcommand{\mapk}{\mathbf{m}_k}
\newcommand{\mapi}{{m}_i}
\newcommand{\mapik}{{m}_{i,k}}
\newcommand{\mapsk}{{m}_{1,k}}
\newcommand{\mapek}{{m}_{\Ncell,k}}
\newcommand{\zhistory}{\mathbf{e}_{1:k}}
\newcommand{\zk}{\mathbf{e}_{k}}
\newcommand{\zkpast}{\mathbf{e}_{k-1}}
\newcommand{\bk}{{b}_{k}}
\newcommand{\bs}{{b}_{0}}
\newcommand{\logoddk}{{\ell}_{k}}
\newcommand{\logoddkprev}{\ell_{k-1}}
\newcommand{\logodds}{\ell_{0}}
% Radar definition
\newcommand{\thetab}{\theta_b}
\newcommand{\Nsteer}{N_{\mathsf{steer}}}
\newcommand{\Nbin}{N_{\mathsf{bins}}}

\newcommand{\xigem}{\xi_m^{(\mathsf{GEM})}}
\newcommand{\xinm}{\xi^{(\mathsf{NM})}}
